Modeling Hierarchical Usage Context for Software Exceptions based on Interaction Data

Traces of user interactions with a software system, captured in production, are commonly used as an input source for user experience testing. In this paper, we present an alternative use, introducing a novel approach of modeling user interaction traces enriched with another type of data gathered in production - software fault reports consisting of software exceptions and stack traces. The model described in this paper aims to improve developers' comprehension of the circumstances surrounding a specific software exception and can highlight specific user behaviors that lead to a high frequency of software faults. Modeling the combination of interaction traces and software crash reports to form an interpretable and useful model is challenging due to the complexity and variance in the combined data source. Therefore, we propose a probabilistic unsupervised learning approach, adapting the Nested Hierarchical Dirichlet Process, which is a Bayesian non-parametric topic model commonly applied to natural language data. This model infers a tree of topics, each of whom describes a set of commonly co-occurring commands and exceptions. The topic tree can be interpreted hierarchically to aid in categorizing the numerous types of exceptions and interactions. We apply the proposed approach to large scale datasets collected from the ABB RobotStudio software application, and evaluate it both numerically and with a small survey of the RobotStudio developers.

==> Makefile <==
PAPER     = paper
LATEX     = pdflatex -halt-on-error
BIBTEX    = bibtex


CLS_FILES = $(shell find . -name "*.cls")
TEX_FILES = $(shell find . -name "*.tex")
BIB_FILES = $(shell find . -name "*.bib")
GFX_FILES = $(shell find ./figures)

DEP_FILES = $(CLS_FILES) $(TEX_FILES) $(BIB_FILES) $(GFX_FILES)

all: $(PAPER).pdf 

.ONESHELL edit:
	make view &> /dev/null
	while true; do \
		sleep 1 && \
		inotifywait -r -e modify,attrib,close_write,move,create,delete . && \
		make; done &> /dev/null &
	$(EDITOR) $(TEX_FILES) && kill %1

$(PAPER).pdf: $(DEP_FILES)
	$(LATEX) $(PAPER) || $(BIBTEX) $(PAPER)
	$(BIBTEX) $(PAPER) || $(LATEX) $(PAPER)
	$(LATEX) $(PAPER) || $(BIBTEX) $(PAPER)
	$(LATEX) $(PAPER)


tidy:
	$(RM) *.aux
	$(RM) *.log
	$(RM) *.out
	$(RM) *.toc
	#$(RM) *.bbl
	$(RM) *.blg

clean: tidy
	$(RM) $(PAPER).pdf $(REVISION).pdf

OS = $(shell uname -s)
ifeq ($(strip $(OS)),Linux)
	PDF_VIEW = xdg-open
else
	PDF_VIEW = open -a /Applications/Preview.app
endif

view: $(PAPER).pdf
	$(PDF_VIEW) $(PAPER).pdf &

